CFDNet: A Generalizable Foggy Stereo Matching Network with Contrastive Feature Distillation

Stereo matching under foggy scenes remains a challenging task since the scattering effect degrades the visibility and results in less distinctive features for dense correspondence matching. While some previous learning-based methods integrated a physical scattering function for simultaneous stereo-matching and dehazing, simply removing fog might not aid depth estimation because the fog itself can provide crucial depth cues. In this work, we introduce a framework based on contrastive feature distillation (CFD). This strategy combines feature distillation from merged clean-fog features with contrastive learning, ensuring balanced dependence on fog depth hints and clean matching features. This framework helps to enhance model generalization across both clean and foggy environments. Comprehensive experiments on synthetic and real-world datasets affirm the superior strength and adaptability of our method.

==> Introduction.tex <==
% Introduction
\section{Introduction}
% Stereo Matching is a fundamental computer vision task, which uses the disparity information of the left and right images to infer depth. Owing to the affordability of stereo cameras, stereo matching is widely used in domains such as Augmented Reality (AR), Virtual Reality (VR), and autonomous driving. However, in practical situations, particularly in autonomous driving scenarios, the presence of adverse weather conditions such as fog or haze is quite common. Under such circumstances, image visibility is substantially diminished, which brings great challenges to stereo matching. Learning-based stereo-matching networks~\cite{gwcnet,dispnetc,ganet,RaftStereo,psmnet} which are usually pre-trained in clean images show big performance degradation on foggy days, as shown in Figure \ref{fig:FogDegragation}.  

Stereo matching is a crucial task, where depth is inferred using the disparity between left and right images. Given the affordability of stereo cameras, this technique is popular in fields like Augmented Reality (AR), and autonomous driving. However, in practical situations, especially in the context of autonomous driving, adverse weather conditions such as fog or haze are common. These conditions significantly reduce image clarity, posing challenges for stereo matching. Notably, learning-based stereo-matching networks, typically trained on clean images, exhibit apparent performance degradation in foggy conditions, as illustrated in Fig. \ref{fig:FogDegragation}.

% Previous methods~\cite{BidNet,HazeStereoRefinement,CAT} utilize designed networks to counteract the impact of fog on matching by restoring the original clean image following the physical atmospheric scattering process~\cite {VisionInBadWeather,SingleImageVisibility,FogVoluming}.
% Prior research~\cite{BidNet,HazeStereoRefinement,CAT} has employed specifically designed networks to mitigate the effects of fog on matching. These networks aim to reconstruct the original, clean image by considering the atmospheric scattering process~\cite{VisionInBadWeather,SingleImageVisibility,FogVoluming}.
% To achieve this, the network is trained to  predict two fog-related hyperparameters: the transmission parameter \textit{T} and the airtightness $L_{\infty}$ within the atmospheric scattering process while estimating the disparity~\cite{FoggyStereo,song2020simultaneous}. 
Prior research~\cite{BidNet,HazeStereoRefinement,CAT} employs networks to mitigate fog's effects on matching by reconstructing the clean image using the atmospheric scattering process~\cite{VisionInBadWeather,SingleImageVisibility,FogVoluming}. These networks simultaneously predict two fog-related hyperparameters: the transmission parameter \textit{T} and the airlight $L_{\infty}$, while estimating disparity~\cite{FoggyStereo,song2020simultaneous}.
\begin{figure}[!t]
    \centering
\includegraphics[width=1.0\linewidth]{Figures/KITTI_Degradations.pdf}
    \caption{Clean and Foggy left images from stereo image pairs (top), and estimated disparity maps from each pair with state-of-the-art RaftStereo\cite{RaftStereo} (bottom).} 
    \label{fig:FogDegragation}
    \vspace{-5mm}
\end{figure}
% However, estimating the scattering hyperparameters is a very challenging task. According to the atmospheric scattering function, the transmission and depth exhibit an exponential relationship. Even minor inaccuracies in transmission estimation can lead to cumulative error in disparity estimation, which makes the whole training unstable and lacks generalization ability in real-world applications. 
Estimating scattering hyperparameters is challenging with the exponential relationship between transmission and depth. Small errors in transmission estimation can result in significant disparity errors, making training unstable and less generalizable in real-world scenarios.

% Different from the existing physical prior-based stereo-matching methods at haze conditions trying to improve performance by pixel-level dehazing, in this paper, we center on directly extracting enhanced matching feature representations from images to improve the performance of stereo matching in different conditions using distilling and contrastive learning strategy and proposed a network named \textit{DCNet}. The intuitive observation comes from that the haze image itself is not always harmful for stereo matching since the thickness of the fog contains depth hints which is beneficial for disparity refinement from a mono-depth aspect. (1)We first proposed a feature converter that consists of stacked pixel-wise and channel-wise attention for adaptive feature fusion from paired clean-haze image inputs. (2)Then we regard such a network as the \textit{Teacher Model} to provide feature-level guidance to distilling the \textit{Student Model} with the same architecture but only haze or clean image as the input. (3)To further prevent the network from relying too much on the features of foggy images for depth estimation during the learning, in addition to distilling loss, we also designed a contrastive loss by pulling in the distance between the feature extracted from the haze images and the feature extracted from the clean images after distillation, while pulling away the distance from the original haze feature which does not enter the feature converter module. (4) We conducted extensive experiments on both synthetic and real-world scenarios such as SceneFlow~\cite{dispnetc}, KITTI~\cite{KITTIDatset}, and PixelAccurateDepeth~\cite{PixelAccurateDepth} datasets following the proposed pipeline with distilling and contrastive loss. Our proposed \textit{DCNet} outperforms the state-of-the-art approaches in both foggy and clean scenes, which fully demonstrates the effectiveness and practicality of our proposed method.

In contrast to physical prior-based stereo-matching methods for hazy conditions that combine image dehazing, this paper emphasizes enhancing matching feature representations from both clean and hazy images to boost stereo matching across varying conditions. We propose a contrastive feature distillation~(CFD) strategy and a network named \textit{CFDNet}. Surprisingly, we discovered that fog does not invariably degrade stereo matching. The fog's thickness can offer valuable depth cues, where we demonstrate its effectiveness in enhancing matching features significantly with our contrastive feature distillation. Our contributions are summarized as follows:
%  help refine disparity from a mono-depth perspective. Our contributions can be summarized as follows:

\begin{itemize}
    % \item Contrast-Balanced Distillation: we integrate contrastive learning into the distillation process to balance distilled feature representation across clean and haze domains. Based on this, we propose a teacher-student model to achieve robust performance across both clean and haze domains by balancing the features' dependence on fog depth hints and clean matching features.
    \item Contrastive Learning Incorporated Feature Distillation: We incorporate contrastive learning into feature distillation, ensuring a balanced distilled feature representation between clean and hazy domains. Based on this, we introduce a teacher-student model that optimizes performance across both domains by harmonizing reliance on fog depth cues with clean matching features.
    % We propose a \textit{Teacher Model} that merges features from clean and hazy images features processed by the feature converter. Despite its dual-input design preventing inference, it guides the \textit{Student Model}, which shares the similar architecture and can infer with either hazy or clean images. For robust performance across both haze and clean domains, a contrastive loss is introduced, balancing the features' dependence on fog depth hints and clean matching features.
    % pulling in the distance between the feature extracted from the haze images and the feature extracted from the clean images after distillation, while pulling away the distance from the original haze feature which does not enter the feature converter module
    \item Attentive Feature Converter: We proposed an attentive feature converter with stacked pixel and channel-wise attention. It enables fine-grained feature fusion for the \textit{Teacher Model} and feature adaptation for \textit{Student Model} with proposed contrastive feature distillation framework.
    \item We conducted comprehensive experiments in both synthetic and real-world settings, utilizing datasets including SceneFlow~\cite{dispnetc}, KITTI~\cite{KITTIDatset}, and PixelAccurateDepeth~\cite{PixelAccurateDepth}. Proposed \textit{CFDNet} surpasses leading methods in both foggy and clean environments, underlining its strong efficacy and applicability. We will open-source the related code and synthetic foggy stereo dataset.
\end{itemize}


